Graph Summarization via Node Grouping: A Spectral Algorithm

Graph summarization via node grouping is a popular method to build concise graph representations by grouping nodes from the original graph into supernodes and encoding edges into superedges such that the loss of adjacency information is minimized. Such summaries have immense applications in large-scale graph analytics due to their small size and high query processing efficiency. In this paper, we reformulate the loss minimization problem for summarization into an equivalent integer maximization problem. By initially allowing relaxed (fractional) solutions for integer maximization, we analytically expose the underlying connections to the spectral properties of the adjacency matrix. Consequently, we design an algorithm called SpecSumm that consists of two phases. In the first phase, motivated by spectral graph theory, we apply k-means clustering on the k largest (in magnitude) eigenvectors of the adjacency matrix to assign nodes to supernodes. In the second phase, we propose a greedy heuristic that updates the initial assignment to further improve summary quality. Finally, via extensive experiments on 11 datasets, we show that SpecSumm efficiently produces high-quality summaries compared to state-of-the-art summarization algorithms and scales to graphs with millions of nodes.

==> integer_baselines_compare.tex <==
\begin{figure*}[ht]
	\captionsetup{skip=3pt}
	\captionsetup[sub]{skip=0pt}
	\centering
	\includegraphics[width=0.9\textwidth]{fig/legend_integer_baselines_objval.pdf}
	% \includegraphics[width=0.6\textwidth]{fig/legend_integer_baselines_objval.pdf}
	\\
	\vspace{3pt}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/SBM_integer_baselines_objval.pdf}
	  \caption{\sbm}
	  \label{fig:SBM_integer_trace}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/Cora_integer_baselines_objval.pdf}
	  \caption{\cora}
	  \label{fig:Cora_integer_trace}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/PPI_integer_baselines_objval.pdf}
	  \caption{\PPI}
	  \label{fig:PPI_integer_trace}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/caGrQc_integer_baselines_objval.pdf}
		\caption{\caGrQc}
	\label{fig:caGrQc_integer_trace}
	\end{subfigure}
	  \\
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/LastFM_Asia_integer_baselines_objval.pdf}
		\caption{\lastfm}
		\label{fig:LastFM_Asia_integer_trace}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/Blogcatalog_integer_baselines_objval.pdf}
		\caption{\blogcatalog}
	\label{fig:Blogcatalog_integer_trace}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/PPI_integer_baselines_objval.pdf}
		% \includegraphics[width=\textwidth]{fig/Facebook_integer_baselines_objval.pdf}
		\caption{\facebook}
	\label{fig:Facebook_integer_trace}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/caGrQc_integer_baselines_objval.pdf}
		% \includegraphics[width=\textwidth]{fig/Email_Enron_integer_baselines_objval.pdf}
		\caption{\enron}
	\label{fig:Email_Enron_integer_trace}
	\end{subfigure}
	\caption{Comparing Integer Baselines.}
	\label{fig:integer_baselines_trace_objval}
	\Description{Experiment 1}
  \end{figure*}
  

==> plot_large_graph_runtimes.tex <==
\begin{figure*}[ht]
	\captionsetup{skip=3pt}
	\captionsetup[sub]{skip=0pt}
	\centering
	% \includegraphics[width=0.9\textwidth]{fig/legend_total_runtimes.pdf}
	% \\
	% \vspace{3pt}
	\begin{subfigure}{0.32\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/Amazon_runtime.pdf}
	  \caption{\Amazon}
	  \label{fig:Amazon_runtime}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/Youtube_runtime.pdf}
	  \caption{\Youtube}
	  \label{fig:Youtube_runtime}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/Wikitalk_runtime.pdf}
	  \caption{\Wikitalk}
	  \label{fig:Wikitalk_runtime}
	\end{subfigure}
	\caption{Blah.}
	\label{fig:large_graph_runtime}
	\Description{Experiment 6}
  \end{figure*}
  

==> plot_relaxed_baselines_first_term_compare.tex <==
\begin{figure*}[ht]
	\captionsetup{skip=3pt}
	\captionsetup[sub]{skip=0pt}
	\centering
	\includegraphics[width=0.9\textwidth]{fig/legend_relaxed_baselines_objval.pdf}
	\\
	\vspace{3pt}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/SBM_relaxed_baselines_First_Term.pdf}
	  \caption{\sbm}
	  \label{fig:SBM_relaxed_trace_T_1}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/Cora_relaxed_baselines_First_Term.pdf}
	  \caption{\cora}
	  \label{fig:Cora_relaxed_trace_T_1}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/PPI_relaxed_baselines_First_Term.pdf}
	  \caption{\PPI}
	  \label{fig:PPI_relaxed_trace_T_1}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/caGrQc_relaxed_baselines_First_Term.pdf}
		\caption{\caGrQc}
	\label{fig:caGrQc_relaxed_trace_T_1}
\end{subfigure}
	  \\
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/LastFM_Asia_relaxed_baselines_First_Term.pdf}
		\caption{\lastfm}
		\label{fig:LastFM_Asia_relaxed_trace_T_1}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/Blogcatalog_relaxed_baselines_First_Term.pdf}
		\caption{\blogcatalog}
	\label{fig:Blogcatalog_relaxed_trace_T_1}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/Facebook_relaxed_baselines_First_Term.pdf}
		\caption{\facebook}
	\label{fig:Facebook_relaxed_trace_T_1}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/Email_Enron_relaxed_baselines_First_Term.pdf}
		\caption{\enron}
	\label{fig:Email_Enron_relaxed_trace_T_1}
	\end{subfigure}
	\caption{First term ($T_1$) of the relaxed objective value ($\FZ{\Z{}}$) in Problem~\ref{prob:trace_maximization_relaxed} (relaxed case) as a function of summary size \summarysize for variants of \lmeigvecs and \opt.}
	\label{fig:relaxed_baselines_first_term}
  \end{figure*}
  

==> plot_relaxed_baselines_second_term_compare.tex <==
\begin{figure*}[ht]
	\captionsetup{skip=3pt}
	\captionsetup[sub]{skip=0pt}
	\centering
	\includegraphics[width=0.9\textwidth]{fig/legend_relaxed_baselines_objval.pdf}
	\\
	\vspace{3pt}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/SBM_relaxed_baselines_Second_Term.pdf}
	  \caption{\sbm}
	  \label{fig:SBM_relaxed_trace_T_2}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/Cora_relaxed_baselines_Second_Term.pdf}
	  \caption{\cora}
	  \label{fig:Cora_relaxed_trace_T_2}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
	  \centering
	  \includegraphics[width=\textwidth]{fig/PPI_relaxed_baselines_Second_Term.pdf}
	  \caption{\PPI}
	  \label{fig:PPI_relaxed_trace_T_2}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/caGrQc_relaxed_baselines_Second_Term.pdf}
		\caption{\caGrQc}
	\label{fig:caGrQc_relaxed_trace_T_2}
\end{subfigure}
	  \\
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/LastFM_Asia_relaxed_baselines_Second_Term.pdf}
		\caption{\lastfm}
		\label{fig:LastFM_Asia_relaxed_trace_T_2}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/Blogcatalog_relaxed_baselines_Second_Term.pdf}
		\caption{\blogcatalog}
	\label{fig:Blogcatalog_relaxed_trace_T_2}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/Facebook_relaxed_baselines_Second_Term.pdf}
		\caption{\facebook}
	\label{fig:Facebook_relaxed_trace_T_2}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{fig/Email_Enron_relaxed_baselines_Second_Term.pdf}
		\caption{\enron}
	\label{fig:Email_Enron_relaxed_trace_T_2}
	\end{subfigure}
	\caption{Second term ($T_2$) of the relaxed objective value ($\FZ{\Z{}}$) in Problem~\ref{prob:trace_maximization_relaxed} (relaxed case) as a function of summary size \summarysize for variants of \lmeigvecs and \opt.}
	\label{fig:relaxed_baselines_second_term}
  \end{figure*}
  

==> tables/Cora_integer_baseline_compare.tex <==
\begin{table}[t!]

		% \setlength\tabcolsep{4pt}

		% \fontsize{8}{6}

		\fontsize{8.5}{8.4}\selectfont 

		\centering 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                    0.02 &                    0.02 &                    0.02 &                    0.03 &                    0.03 &                    0.04 \\
                              \textsc{S2L} &                    0.22 &                    0.42 &                     0.7 &                    0.89 &                    0.94 &                    1.05 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    0.32 &                    0.85 &                    1.09 &                     1.3 &                    1.37 &         \underline{1.6} \\
                         \textsc{SpecSumm} &        \underline{0.49} &        \underline{0.86} &        \underline{1.25} &        \underline{1.49} &        \underline{1.43} &                    1.59 \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}0.51 & \cellcolor{blue!25}0.91 & \cellcolor{blue!25}1.29 & \cellcolor{blue!25}1.55 & \cellcolor{blue!25}1.52 & \cellcolor{blue!25}1.68 \\
\bottomrule 
 \end{tabular} 
\caption{Objective value ($\mathcal{F}_{Z}$) of Problem 1 (integer) for \textsc{Cora}. Blue denotes best performance.}
\label{tab:Cora_integer_baselines}
\end{table}

==> tables/PPI_integer_baseline_compare.tex <==
\begin{table}[t!]

		% \setlength\tabcolsep{4pt}

		% \fontsize{8}{6}

		\fontsize{8.5}{8.4}\selectfont 

		\centering 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                     0.4 &                   0.43 &                     0.45 &                      0.5 &                     0.5 &                     0.57 \\
                              \textsc{S2L} &                    5.18 &                   5.49 &                     6.58 &                     7.09 &                    6.99 &                     7.26 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    3.78 &                   5.09 &                     5.11 &                     5.22 &                    5.64 &                     5.43 \\
                         \textsc{SpecSumm} &        \underline{6.23} &        \underline{8.0} &         \underline{9.65} &         \underline{9.94} &       \underline{10.01} &        \underline{10.49} \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}6.79 & \cellcolor{blue!25}8.7 & \cellcolor{blue!25}10.27 & \cellcolor{blue!25}10.49 & \cellcolor{blue!25}10.7 & \cellcolor{blue!25}11.27 \\
\bottomrule 
 \end{tabular} 
\caption{Objective value ($\mathcal{F}_{Z}$) of Problem 1 (integer) for \textsc{PPI}. Blue denotes best performance.}
\label{tab:PPI_integer_baselines}
\end{table}

==> tables/appd_integer_baseline_compare.tex <==
\begin{table*}[t!]

		\setlength\tabcolsep{4pt}

		% \fontsize{8}{6}

		\fontsize{8.5}{8.3}\selectfont 

	\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                    3.57 &                    3.57 &                    3.58 &                    3.59 &                     3.6 &                    3.62 \\
                              \textsc{S2L} &                    3.57 &                    3.59 &                    3.61 &                    3.62 &                    3.63 &                    3.64 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    3.73 &                    3.79 &                    3.86 &                     3.9 &                    3.93 &                    4.12 \\
                         \textsc{SpecSumm} &        \underline{3.88} &        \underline{4.22} &        \underline{4.56} &        \underline{4.89} &        \underline{5.08} &        \underline{5.11} \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}3.92 & \cellcolor{blue!25}4.31 & \cellcolor{blue!25}4.69 & \cellcolor{blue!25}5.03 & \cellcolor{blue!25}5.23 & \cellcolor{blue!25}5.28 \\
\bottomrule 
 \end{tabular} 
\caption{\textsc{SBM}}
\end{subtable}% 
\hfill 
\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                   0.04 &                    0.05 &                    0.05 &                    0.06 &                    0.06 &                    0.06 \\
                              \textsc{S2L} &                   5.56 &                    7.03 &                    7.48 &                    7.17 &        \underline{8.14} &                    8.15 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    6.0 &                    6.87 & \cellcolor{blue!25}7.83 & \cellcolor{blue!25}7.96 & \cellcolor{blue!25}8.88 & \cellcolor{blue!25}8.81 \\
                         \textsc{SpecSumm} &       \underline{6.58} &        \underline{7.33} &                     7.7 &                    7.65 &                    7.85 &                    8.41 \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}6.6 & \cellcolor{blue!25}7.36 &        \underline{7.79} &         \underline{7.8} &                     8.0 &        \underline{8.64} \\
\bottomrule 
 \end{tabular} 
\caption{\textsc{ca-GrQc}}
\end{subtable}% 
\par\bigskip 
\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                    0.05 &                    0.06 &                    0.06 &                    0.06 &                    0.06 &                   0.07 \\
                              \textsc{S2L} &                    3.34 &                    4.22 &                    5.01 &                    5.33 &                    6.02 &                   6.22 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    3.62 &                    4.89 &                    5.87 & \cellcolor{blue!25}6.87 &        \underline{7.69} & \cellcolor{blue!25}8.3 \\
                         \textsc{SpecSumm} &        \underline{3.91} &        \underline{5.27} &        \underline{6.25} &                    6.76 &                    7.54 &                   7.98 \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}3.94 & \cellcolor{blue!25}5.34 & \cellcolor{blue!25}6.32 &        \underline{6.85} & \cellcolor{blue!25}7.71 &       \underline{8.14} \\
\bottomrule 
 \end{tabular} 
\caption{\textsc{LastFM-Asia}}
\end{subtable}% 
\hfill 
\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                      4.3 &                       4.4 &                     4.68 &                      4.5 &                      4.76 &                      4.69 \\
                              \textsc{S2L} & \cellcolor{blue!25}96.52 & \cellcolor{blue!25}105.66 & \cellcolor{blue!25}108.9 &                   112.03 &                    113.62 &                    112.31 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    58.14 &                     59.56 &       \underline{106.68} & \cellcolor{blue!25}114.8 &                    110.03 & \cellcolor{blue!25}121.23 \\
                         \textsc{SpecSumm} &                    86.07 &                    100.78 &                   100.81 &                   112.85 &        \underline{116.07} &                    116.83 \\
              \textsc{SpecSumm}-\textsc{R} &        \underline{87.25} &        \underline{102.54} &                    102.7 &       \underline{114.56} & \cellcolor{blue!25}117.76 &        \underline{118.75} \\
\bottomrule 
 \end{tabular} 
\caption{\textsc{Blogcatalog}}
\end{subtable}% 
\par\bigskip 
\caption{Objective value, $\mathcal{F}_{Z}$ ($\times 10^3$), of Problem 1 (integer) for \textsc{SBM}, \textsc{ca-GrQc}, \textsc{LastFM-Asia}, and \textsc{Blogcatalog}. Values highlighted in blue denote best performance and underlined values denote second-best performance.}
\label{tab:main_integer_baselines}
\end{table*}

==> tables/graph_query_estimate.tex <==
\begin{table*}[t]

		\captionsetup[sub]{skip=0pt} 

		\centering  

		\footnotesize 

		\setlength\tabcolsep{4pt} 

		\caption{The trace objective value, $\mathcal{F}_{Z}$ ($ \times 10^3$), of Problem 1 for the summaries computed by each algorithm across different datasets. The values highlighted in blue denote the best quality and the underlined values denote the second-best quality.}
		\label{tab:main_integer_baselines} 

		\vspace{-1em} 

		\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	

==> tables/large_graphs_objvals.tex <==
\begin{table*}[t!]

		\setlength\tabcolsep{3pt}

		\setlength\extrarowheight{1.5pt}

		% \fontsize{8}{6}

		\fontsize{7.5}{8.0}\selectfont 

	\begin{subtable}{.3\linewidth}% 

		\centering% 

		\begin{tabular}{ccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Eigenvectors}} & \multirow{2}[2]{*}{\textbf{$k$}} & \multicolumn{2}{c}{\textbf{Objective ($\times 10^{3}$)}} & \multirow{2}[2]{*}{\textbf{Runtime}} \\ 

		\cmidrule(lr){3-4} 

		& & $\mathcal{F}_{Z}$ & $\text{L}_{\text{norm}}$ & \\ 

		\midrule 

	\multirow{6}{*}{100} & 100  &             4.572 &                    1.359 &   0.089 \\
      & 250  &            10.286 &                    1.357 &   0.226 \\
      & 500  &            13.891 &                    1.356 &    0.77 \\
      & 1000 &            21.062 &                    1.353 &   0.617 \\
      & 2000 &            30.071 &                     1.35 &   3.092 \\
      & 5000 &            48.253 &                    1.343 &   3.344 \\
 \cline{1-5}
 \multirow{6}{*}{250} & 100  &              3.74 &                    1.359 &   0.233 \\
      & 250  &            10.768 &                    1.357 &   0.677 \\
      & 500  &            19.278 &                    1.354 &   0.762 \\
      & 1000 &            34.274 &                    1.348 &   1.398 \\
      & 2000 &            44.486 &                    1.344 &   2.446 \\
      & 5000 &            67.263 &                    1.336 &   9.433 \\
 \cline{1-5}
 \multirow{6}{*}{500} & 100  &             3.707 &                    1.359 &   0.545 \\
      & 250  &            10.308 &                    1.357 &    1.07 \\
      & 500  &            20.631 &                    1.353 &   1.092 \\
      & 1000 &            40.921 &                    1.346 &   2.418 \\
      & 2000 &            63.879 &                    1.337 &   4.072 \\
      & 5000 &            91.881 &                    1.327 &  14.022 \\
 \cline{1-5}
 \multirow{6}{*}{1000} & 100  &             3.518 &                    1.359 &   2.484 \\
      & 250  &             9.106 &                    1.357 &   3.341 \\
      & 500  &            19.423 &                    1.354 &   3.739 \\
      & 1000 &            40.385 &                    1.346 &    6.97 \\
      & 2000 &            74.006 &                    1.333 &  10.789 \\
      & 5000 &           126.961 &                    1.313 &  29.867 \\
 \cline{1-5}
 \multirow{5}{*}{2000} & 100  &             3.242 &                     1.36 &   6.852 \\
      & 250  &             8.095 &                    1.358 &   8.018 \\
      & 500  &            17.068 &                    1.354 &   10.21 \\
      & 1000 &            36.011 &                    1.347 &  13.431 \\
      & 2000 &            76.083 &                    1.333 &  20.385 \\
 \cline{1-5}
 100  & 100  &             9.037 &                    1.357 &   0.012 \\
 250  & 250  &             9.199 &                    1.357 &   0.013 \\
 500  & 500  &            25.229 &                    1.351 &   0.016 \\
 1000 & 1000 &             25.28 &                    1.351 &   0.013 \\
 2000 & 2000 &            64.518 &                    1.337 &   0.013 \\
 5000 & 5000 &           154.103 &                    1.303 &   0.013 \\

\bottomrule 
 \end{tabular} 
\caption{\textsc{Amazon}}
\end{subtable}% 
\hfill 
\begin{subtable}{.3\linewidth}% 

		\centering% 

		\begin{tabular}{ccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Eigenvectors}} & \multirow{2}[2]{*}{\textbf{$k$}} & \multicolumn{2}{c}{\textbf{Objective ($\times 10^{3}$)}} & \multirow{2}[2]{*}{\textbf{Runtime}} \\ 

		\cmidrule(lr){3-4} 

		& & $\mathcal{F}_{Z}$ & $\text{L}_{\text{norm}}$ & \\ 

		\midrule 

	\multirow{6}{*}{100} & 100  &            45.952 &                    2.435 &   0.721 \\
      & 250  &            99.003 &                    2.424 &   0.559 \\
      & 500  &           132.909 &                    2.417 &   1.012 \\
      & 1000 &           184.095 &                    2.406 &   2.249 \\
      & 2000 &           357.422 &                     2.37 &   5.244 \\
      & 5000 &           554.563 &                    2.328 &  15.948 \\
 \cline{1-5}
 \multirow{6}{*}{250} & 100  &             30.56 &                    2.438 &    0.52 \\
      & 250  &            55.211 &                    2.433 &   1.315 \\
      & 500  &           120.893 &                     2.42 &    1.83 \\
      & 1000 &           229.617 &                    2.397 &   4.019 \\
      & 2000 &           293.012 &                    2.384 &   7.217 \\
      & 5000 &           396.752 &                    2.362 &  23.967 \\
 \cline{1-5}
 \multirow{5}{*}{500} & 100  &             15.94 &                    2.441 &   1.702 \\
      & 250  &            27.172 &                    2.439 &    3.01 \\
      & 500  &            55.931 &                    2.433 &   3.277 \\
      & 1000 &           174.641 &                    2.408 &   5.916 \\
      & 2000 &           299.588 &                    2.382 &  18.129 \\
 \cline{1-5}
 \multirow{5}{*}{1000} & 100  &             5.806 &                    2.443 &    4.32 \\
      & 250  &             12.01 &                    2.442 &   6.906 \\
      & 500  &            19.576 &                     2.44 &   8.055 \\
      & 1000 &            80.058 &                    2.428 &  15.713 \\
      & 2000 &           270.582 &                    2.388 &  28.823 \\
 \cline{1-5}
 \multirow{3}{*}{2000} & 100  &             2.603 &                    2.444 &  14.165 \\
      & 250  &             6.076 &                    2.443 &  18.269 \\
      & 500  &             9.515 &                    2.442 &  21.361 \\
 \cline{1-5}
 100  & 100  &            45.504 &                    2.435 &    0.17 \\
 250  & 250  &            46.625 &                    2.435 &   0.166 \\
 500  & 500  &           111.331 &                    2.422 &   0.169 \\
 1000 & 1000 &           110.069 &                    2.422 &   0.188 \\
 2000 & 2000 &           223.527 &                    2.398 &   0.195 \\
 5000 & 5000 &           296.653 &                    2.383 &   0.171 \\

\bottomrule 
 \end{tabular} 
\caption{\textsc{Youtube}}
\end{subtable}% 
\hfill 
\begin{subtable}{.3\linewidth}% 

		\centering% 

		\begin{tabular}{ccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Eigenvectors}} & \multirow{2}[2]{*}{\textbf{$k$}} & \multicolumn{2}{c}{\textbf{Objective ($\times 10^{3}$)}} & \multirow{2}[2]{*}{\textbf{Runtime}} \\ 

		\cmidrule(lr){3-4} 

		& & $\mathcal{F}_{Z}$ & $\text{L}_{\text{norm}}$ & \\ 

		\midrule 

	\multirow{6}{*}{100} & 100  &            67.438 &                    3.041 &   0.569 \\
      & 250  &           272.607 &                    3.007 &    1.17 \\
      & 500  &           150.137 &                    3.027 &   3.302 \\
      & 1000 &           450.756 &                    2.977 &   4.456 \\
      & 2000 &           490.885 &                     2.97 &  15.822 \\
      & 5000 &           898.972 &                    2.901 &  25.105 \\
 \cline{1-5}
 \multirow{5}{*}{250} & 100  &            26.396 &                    3.047 &    1.37 \\
      & 250  &            79.794 &                    3.039 &   2.639 \\
      & 500  &           120.674 &                    3.032 &     4.1 \\
      & 1000 &           236.116 &                    3.013 &   8.753 \\
      & 2000 &           533.634 &                    2.963 &  20.895 \\
 \cline{1-5}
 \multirow{4}{*}{500} & 100  &             0.689 &                    3.052 &   3.169 \\
      & 250  &            19.261 &                    3.049 &   5.523 \\
      & 500  &            45.983 &                    3.044 &   7.749 \\
      & 1000 &           111.779 &                    3.033 &  11.853 \\
 \cline{1-5}
 \multirow{4}{*}{1000} & 100  &              0.54 &                    3.052 &   6.801 \\
      & 250  &             0.754 &                    3.052 &  10.449 \\
      & 500  &             9.413 &                     3.05 &  14.463 \\
      & 1000 &            89.058 &                    3.037 &  34.754 \\
 \cline{1-5}
 \multirow{3}{*}{2000} & 100  &              0.28 &                    3.052 &  23.127 \\
      & 250  &             0.452 &                    3.052 &  31.885 \\
      & 500  &             1.319 &                    3.052 &  38.458 \\
 \cline{1-5}
 100  & 100  &           105.996 &                    3.034 &   0.339 \\
 250  & 250  &           103.321 &                    3.035 &   0.386 \\
 500  & 500  &           268.151 &                    3.008 &   0.415 \\
 1000 & 1000 &           599.605 &                    2.952 &   0.325 \\
 2000 & 2000 &           594.372 &                    2.953 &   0.344 \\
 5000 & 5000 &           862.636 &                    2.907 &   0.347 \\

\bottomrule 
 \end{tabular} 
\caption{\textsc{Wikitalk}}
\end{subtable}% 
\hfill 
\caption{Trade-off between number of eigenvectors and size of summary ($k$) on the integer objective values ($\mathcal{F}_{Z}$) and $\text{L}_{\text{norm}}$) for \textsc{Amazon}, \textsc{Youtube}, and \textsc{Wikitalk}. Good quality summaries of larger sizes may be constructed from fewer eigenvectors, but smaller summaries constructed from higher number of eigenvectors are poorer in quality.}
\label{tab:large_datasets_integer_baselines}
\end{table*}

==> tables/main_integer_baseline_compare.tex <==
\begin{table*}[t!]

		\setlength\tabcolsep{4pt}

		% \fontsize{8}{6}

		\fontsize{8.5}{8.3}\selectfont 

	\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                    0.02 &                    0.02 &                   0.02 &                   0.03 &                    0.03 &                   0.04 \\
                              \textsc{S2L} &                    0.22 &                    0.42 &                    0.7 &                   0.89 &                    0.94 &                   1.05 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    0.32 &                    0.85 &                   1.09 &                    1.3 &                    1.37 &        \underline{1.6} \\
                         \textsc{SpecSumm} &        \underline{0.49} &        \underline{0.86} &       \underline{1.25} &       \underline{1.48} &        \underline{1.43} &                   1.59 \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}0.58 & \cellcolor{blue!25}1.03 & \cellcolor{blue!25}1.4 & \cellcolor{blue!25}1.7 & \cellcolor{blue!25}1.72 & \cellcolor{blue!25}1.9 \\
\bottomrule 
 \end{tabular} 
\caption{\textsc{Cora}}
\end{subtable}% 
\hfill 
\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                     0.4 &                   0.43 &                     0.45 &                      0.5 &                      0.5 &                     0.57 \\
                              \textsc{S2L} &                    5.18 &                   5.49 &                     6.58 &                     7.09 &                     6.99 &                     7.26 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    3.78 &                   5.09 &                     5.11 &                     5.22 &                     5.64 &                     5.43 \\
                         \textsc{SpecSumm} &        \underline{6.23} &        \underline{8.0} &         \underline{9.65} &         \underline{9.94} &        \underline{10.01} &        \underline{10.49} \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}7.38 & \cellcolor{blue!25}9.6 & \cellcolor{blue!25}11.23 & \cellcolor{blue!25}11.92 & \cellcolor{blue!25}12.22 & \cellcolor{blue!25}12.96 \\
\bottomrule 
 \end{tabular} 
\caption{\textsc{PPI}}
\end{subtable}% 
\par\bigskip 
\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                     0.23 &                     0.24 &                     0.24 &                     0.24 &                    0.24 &                     0.25 \\
                              \textsc{S2L} &                    17.62 &                    31.64 &                    39.35 &                    45.66 &                   51.56 &                     57.2 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    20.05 &                    34.25 & \cellcolor{blue!25}50.16 &                    54.24 &       \underline{59.77} & \cellcolor{blue!25}64.32 \\
                         \textsc{SpecSumm} &        \underline{26.96} &         \underline{40.7} &                    49.04 &        \underline{54.26} &                   59.65 &                    63.48 \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}27.16 & \cellcolor{blue!25}40.95 &        \underline{49.33} & \cellcolor{blue!25}54.64 & \cellcolor{blue!25}60.1 &         \underline{64.0} \\
\bottomrule 
 \end{tabular} 
\caption{\textsc{Facebook}}
\end{subtable}% 
\hfill 
\begin{subtable}{.485\linewidth}% 

		\centering% 

		\begin{tabular}{lcccccc} 

		\toprule 

		\multirow{2}[2]{*}{\textbf{Algorithm}} & \multicolumn{6}{c}{\textbf{$k$ (Summary Size)}} \\ 

		\cmidrule(lr){2-7} 

		& $20$ & $40$ & $60$ & $80$ & $100$ & $120$ \\ 

		\midrule 

	                           \textsc{Random} &                    0.12 &                     0.12 &                     0.13 &                     0.13 &                     0.12 &                     0.13 \\
                              \textsc{S2L} &                   16.92 & \cellcolor{blue!25}23.36 & \cellcolor{blue!25}25.99 & \cellcolor{blue!25}27.76 &        \underline{29.23} &                    31.57 \\
\textsc{DeepWalk}-\textsc{Opt}-\textsc{KM} &                    14.2 &                    15.77 &                     19.4 &                    23.71 &                    24.16 &                     26.3 \\
                         \textsc{SpecSumm} &       \underline{17.25} &                     21.0 &                    23.81 &                    27.09 &                    29.02 &        \underline{32.44} \\
              \textsc{SpecSumm}-\textsc{R} & \cellcolor{blue!25}17.4 &        \underline{21.31} &        \underline{24.09} &        \underline{27.41} & \cellcolor{blue!25}29.43 & \cellcolor{blue!25}32.98 \\
\bottomrule 
 \end{tabular} 
\caption{\textsc{Email-Enron}}
\end{subtable}% 
\par\bigskip 
\caption{Objective value, $\mathcal{F}_{Z}$ ($\times 10^{3}$), of Problem 1 (integer) for \textsc{Cora}, \textsc{PPI}, \textsc{Facebook}, and \textsc{Email-Enron}. Values highlighted in blue denote best performance and underlined values denote second-best performance.}
\label{tab:integer_baselines}
\end{table*}
